LaMini-LM: A Diverse Herd of Distilled Models from Large-Scale Instructions

Large language models (LLMs) with instruction fine-tuning demonstrate superior generative capabilities. However, these models are resource-intensive. To alleviate this issue, we explore distilling knowledge from instruction-tuned LLMs into much smaller ones. To this end, we carefully develop a large set of 2.58M instructions based on both existing and newly-generated instructions. In addition to being sizable, we design our instructions to cover a broad set of topics to ensure diversity. Extensive analysis of our instruction dataset confirms its diversity, and we generate responses for these instructions using gpt-3.5-turbo. Leveraging these instructions, we fine-tune a diverse herd of models, collectively referred to as LaMini-LM, which includes models from both the encoder-decoder and decoder-only families, with varying sizes. We evaluate the performance of our models using automatic metrics on 15 different natural language processing (NLP) benchmarks, as well as through human assessment. The results demonstrate that our proposed LaMini-LM models are comparable to competitive baselines, while being much smaller in size.

==> tables/main.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
               & T5     &  \modelname-T5   &  F-T5       & \modelname-F-T5 & C-GPT & \modelname-C & GPT-2  & \modelname-GPT  & LLaMA  &  Alpaca        \\ \cmidrule(rl){2-3} \cmidrule(rl){4-5} \cmidrule(rl){6-7} \cmidrule(rl){8-9} \cmidrule(l){10-11}
\#params.  & \multicolumn{2}{c}{738M} & \multicolumn{2}{c}{783M}           & \multicolumn{2}{c}{1.3B}     & \multicolumn{2}{c}{1.5B} & \multicolumn{2}{c}{7B} \\ \midrule
OpenBookQA     & 32.8   & 36.0            & 31.2          & 34.0               & 29.0         & 34.0          & 32.0   & 39.8            & 42.4   & 43.2          \\
SciQ           & 82.4   & 84.5            & 93.8          & 86.7               & 73.0         & 79.4          & 76.1   & 80.4            & 66.3   & 69.6          \\
RACE           & 31.5   & 32.6            & 40.9          & 32.8               & 30.3         & 32.9          & 33.1   & 39.1            & 39.9   & 42.2          \\
ARC            & 25.4   & 29.0            & 30.7          & 31.8               & 25.3         & 30.3          & 28.5   & 35.8            & 41.4   & 41.8          \\
PIQA           & 55.9   & 67.2            & 72.2          & 70.6               & 66.8         & 66.9          & 70.5   & 71.3            & 77.5   & 76.0          \\
ReCoRD         & 73.1   & 68.7            & 76.7          & 70.4               & 75.0         & 66.3          & 84.4   & 78.5            & 91.4   & 87.4          \\
SST            & 50.2   & 90.3            & 94.0          & 93.1               & 51.3         & 90.3          & 49.1   & 93.5            & 53.0   & 85.8          \\
MRPC           & 34.3   & 71.1            & 82.6          & 77.9               & 68.4         & 71.3          & 63.2   & 76.0            & 68.4   & 74.3          \\
RTE            & 79.8   & 57.0            & 87.4          & 65.0               & 53.1         & 65.7          & 52.3   & 67.9            & 53.4   & 67.1          \\
MultiNLI       & 61.3   & 54.7            & 72.4          & 61.4               & 35.2         & 47.4          & 36.5   & 67.5            & 34.4   & 38.8          \\
MultiNLI (mis) & 63.1   & 55.8            & 72.0          & 61.0               & 35.4         & 49.2          & 37.0   & 69.3            & 35.6   & 39.6          \\
WSC         & 60.4   & 59.0            & 66.7          & 64.1               & 62.3         & 57.1          & 73.3   & 69.6            & 80.6   & 77.3          \\
WinoGrande     & 55.2   & 54.9            & 59.9          & 56.0               & 51.9         & 51.8          & 58.3   & 56.0            & 67.0   & 65.7          \\
WiC            & 49.4   & 50.5            & 64.7          & 63.8               & 50.2         & 50.2          & 49.8   & 52.4            & 50.0   & 57.5          \\
HellaSwag      & 38.9   & 40.6            & 48.7          & 43.7               & 38.4         & 38.7          & 50.9   & 48.3            & 73.0   & 68.7          \\ \midrule
Average        & 52.9   & \textbf{56.8}   & \textbf{66.3} & 60.8               & 49.7         & \textbf{55.4} & 53.0   & \textbf{63.0}   & 58.3   & \textbf{62.3} \\ \bottomrule
\end{tabular}
\caption{
Automatic evaluation results of selected language models on 15 NLP tasks.
``Average'' indicates the micro-average of the individual task results.
The best average results are highlighted in \textbf{bold}.
F-T5 and \modelname-F-T5 indicate Flan-T5 and \modelname-Flan-T5 respectively.
C-GPT and \modelname-C indicate Cerebras-GPT and \modelname-Cerebras respectively. \\
\textbf{Note:} We are using lm-eval-harness to evaluate our performance. Therefore, LLaMA numbers are not supposed to be compared to the original paper since we are using different method of measurement.
}
\label{tab:main}
\end{table*}
